Exact Conditional Score-Guided Generative Modeling for Amortized Inference in Uncertainty Quantification

We propose an efficient framework for amortized conditional inference by leveraging exact conditional score-guided diffusion models to train a non-reversible neural network as a conditional generative model. Traditional normalizing flow methods require reversible architectures, which can limit their expressiveness and efficiency. Although diffusion models offer greater flexibility, they often suffer from high computational costs during inference. To combine the strengths of both approaches, we introduce a two-stage method. First, we construct a training-free conditional diffusion model by analytically deriving an exact score function under a Gaussian mixture prior formed from samples of the underlying joint distribution. This exact conditional score model allows us to efficiently generate noise-labeled data, consisting of initial diffusion Gaussian noise and posterior samples conditioned on various observation values, by solving a reverse-time ordinary differential equation. Second, we use this noise-labeled data to train a feedforward neural network that maps noise and observations directly to posterior samples, eliminating the need for reversibility or iterative sampling at inference time. The resulting model provides fast, accurate, and scalable conditional sampling for high-dimensional and multi-modal posterior distributions, making it well-suited for uncertainty quantification tasks, e.g., parameter estimation of complex physical systems. We demonstrate the effectiveness of our approach through a series of numerical experiments.

==> numerical_examples.tex <==
\section{Numerical Experiments}\label{sec:num}

In this section, we present numerical experiments to demonstrate the ability of the exact score-guided diffusion model to conduct uncertainty quantification for a diverse set of problems. In cases where the system lacks inherent randomness, we simulate uncertainty by adding white noise to the observed data. In our first example, presented in Section~\ref{sec:ex1}, we perform a series of ablation studies to analyze sources of error and assess the effects of parameter selection on approximation accuracy. Section~\ref{sec:20D_2Mode_GMM} presents a 20 dimensional conditional distribution example and Section~\ref{sec:elliptic_PDE} presents a parameter estimation problem for a 2D elliptic PDE.  

\subsection{1D Bimodal Example.}\label{sec:ex1}

We first consider the approximation of a bimodal distribution to assess the accuracy of the method. The problem setting is the following:
\begin{equation}\label{bimodal_example}
    \bX =
\begin{bmatrix}
\bU \\
\bV
\end{bmatrix},\quad  \bV = \bU^2 + \bveps, \quad \bveps \sim \mathcal{N}(0,\sigma_{\rm true}^2), \quad \sigma_{\rm true}^2 = 0.1 \quad \bU \sim \text{Uniform}[-2,2]. 
\end{equation}
We consider a dataset of joint samples $\{(\bu_{k},\bv_{k})\}_{k=1}^K$, where below we consider $K =500$ and $K =5,000$ prior samples. For all tests below, we assume to observe $\by = 1$. We first present the three reference distributions used as benchmarks. 
\subsubsection{GMM Posterior Distribution}
For the purpose of the ablation studies below, we require the GMM posterior $p_{\bX|\bY}(\bx|\by)$ as defined in Eq.~\eqref{eq:bayes_post}. 
% \begin{equation}\label{exact_GMM_reference}
%     p_{\bX|\bY}(\bx|\by) = \sum_{k=1}^K p_{\xi|\bY}(k|\by) \phi(x|\bmu_{k|\bY}, | \bSigma_{k|\bY}).
% \end{equation} 
% The parameters of the components are defined as follows,
% \begin{equation}
% \begin{split}\label{eq:exact_component_updates}
%  & \bmu_{k|\bY} = \bmu_k + \bSigma_k \bH^\top (\bH \bSigma_k \bH^\top + \bSigma_Y)^{-1} (\by - \bH\bmu_k) \\
% &\bSigma_{k|\bY} = \bSigma_k - \bSigma_k \bH^\top (\bH \bSigma_k \bH^\top + \bSigma_{\bY})^{-1} \bH \bSigma_k. 
% \end{split}
% \end{equation}
% and the weights are defined, 
% \begin{equation}\label{eq:exact_weights}    
%     p_{\xi|\bY}(k|\by) = \frac{p_{\bY|\xi}(\by|k)p_{\xi}(k)}{p_{\bY}(\by)}= \frac{\phi(\by|\bH\bmu_k, \bH{\bSigma}_k \bH^T + \bSigma_{\bY})\pi_k}{\sum_{k=1}^K \pi_k p_{\bY|\xi}(\by|k)}.
% \end{equation}
We can compute the marginal density of interest, $p_{\bU|\bY}(\bu|\by)$:
\begin{equation}\label{posterior_distribution_reference}
    p_{\bU|\bY}(\bu|\by) = \sum_{k=1}^K p_{\xi|\bY}(k|\by) \phi(u|\bmu^{u}_{k|\bY}, | \bSigma^{u}_{k|\bY}).
\end{equation} 
In the below studies, we denote this distribution as $ p_{\rm BGMM}(\bu|\by)$. 
\subsubsection{GMM Conditional Distribution}
We also consider the conditional distribution defined in Eq.~\eqref{eq:cond_dist} as a reference distribution,
\begin{equation}\label{conditional_distribution_reference}
    p_{\rm GMM}(\bu|\bv) = \sum_{k=1}^K p_{\xi|\bV}(k|\bv) \phi(u|\bmu^{u}_{k|\bV}, | \bSigma^{u}_{k|\bV}).
\end{equation} 
When $\sigma_{\bY} = 0$, we have $\bY= \bH\bX + \bveps_{\bY} = \bV$ and $p_{\rm BGMM}(\bu|\by) = p_{\rm GMM}(\bu|\bv)$. We denote the conditional distribution as $p_{\rm GMM}(\bu|\bv)$

% Where the weights $p_{\xi|\bV}(k|\bv)$ are determined by:
% \begin{equation}
%     p_{\xi|\bV}(k|\bv) 
%  = \frac{\pi_k \phi(\by| \bmu^v_k, {\bSigma}^v_k)}{\sum_{k=1}^K \pi_k \phi(\by| \bmu^v_k, {\bSigma}^v_k)}
% \end{equation}
% Additionally, the Gaussian Mixture components simplify to $\bmu_k^u$ and $\bSigma_k^u$. We have as the GMM conditional density:
% \begin{equation}\label{direct_marginal_GMM_reference}
%     p_{\rm GMM}(\bu|\bv) = \sum_{k=1}^K p_{\xi|\bV}(k|\bv) \phi(u|\bmu^{u}_{k}, | \bSigma^{u}_{k}).
% \end{equation} 
\subsubsection{Exact Posterior Distribution}
As a third reference distribution, we compute the exact posterior  distribution with the uniform prior distribution $\text{Uniform}[-2,2]$ given by:
\begin{equation} \label{exact_posterior}
p_{\bU|\bV}(\bu|\bv) = \frac{p_{\bV|\bU}(\by|\bv)p_{\bU}(\bu)}{p_{\bV}(\bv)} = \frac{e^{-\frac{(\bv-\bu^2)^2}{2\sigma^2}} \mathbf{1}_{[-2,2]}(\bu)}{\int_{-\infty}^\infty e^{-\frac{(\bv-\bu^2)^2}{2\sigma^2}}d\bu}.
\end{equation}
In the below studies, this is denoted by $p_{\rm exact}(\bu|\bv)$.
\subsubsection{Quantifying Approximation Accuracy}
The forward KL divergence between reference distributions $p_{\rm ref}$ and the approximate distribution obtained by the exact score-guided diffusion model, denoted $p_{\rm diff}$, is given by
\begingroup
\setlength{\abovedisplayskip}{6pt}
\setlength{\belowdisplayskip}{6pt}
\begin{equation}\label{eq_kl} 
D_{\rm KL}(p_{\rm ref} \mid p_{\rm diff}) = \int_{-\infty}^\infty p_{\rm ref}(x)\log\left(\frac{p_{\rm ref}(x)}{p_{\rm diff}(x)}\right)\,dx.
\end{equation}
\endgroup
 
This integral can be approximated using a Riemann sum over a uniform mesh. Given the generated samples, we perform kernel desnity estimation (KDE) to obtain $p_{\rm diff}(x)$.

\titlespacing{\subsubsection}  % target subsubsection spacing
  {0pt}    % left margin
  {1ex}    % space *before* the heading
  {0.7ex}  % space *after* the heading

\subsubsection{Ablation Study: Conditional density accuracy} The goal of this ablation study is to examine the error between reference distributions and the approximate density obtained by the exact score-guided diffusion model. Both marginal datasets $\bU$ and $\bV$ are first normalized using the z-score transformation. 
We first present a table depicting the error described by the following KL divergence values:

\begin{itemize}[leftmargin=15pt]
    \item $D_{KL}(p_{\rm BGMM}(\bu|\by)||p_{\rm diff}(\bu|\by))$, the KL divergence between the marginal of the posterior density defined in Eq.~\eqref{posterior_distribution_reference} and the approximate density obtained via diffusion model. This error comes from the time discretization of the reverse ODE process, solved using forward Euler. Denote this error as $e_{\rm BGMM}$.
    
    \item $D_{KL}(p_{\rm GMM}(\bu|\bv)||p_{\rm diff}(\bu|\by))$, the KL divergence between the GMM conditional density defined in Eq.~\eqref{conditional_distribution_reference} and the approximate density obtained via diffusion model. This error includes the Bayesian error, i.e. the uncertainty introduced by the choice of $\sigma^2_{\bY}$, as well as the error from the time discretization of the reverse ODE process. Denote this error as $e_{\rm GMM}$.
    
    \item $D_{KL}(p_{\rm exact}(\bu|\bv)||p_{\rm diff}(\bu|\by))$, the KL divergence between the exact posterior distribution defined in Eq.~\eqref{exact_posterior} and the approximate density obtained via diffusion model. This error comes from Bayesian error, time discretization of the reverse ODE process, as well as the approximation accuracy of the exact score-guided diffusion model, which is determined by the number of available prior samples $K$, and selection of $\sigma^2_{\bU}$ and $\sigma^2_{\bV}$ parameter values. Denote this error as $e_{\rm exact}$.
\end{itemize}
\newpage
In the below table we fix $\sigma^2_{\bU} = \sigma^2_{\bV}$ and vary $\sigma^2_{\bY}$:

\vspace{0.5em} 
\begin{center}
\begin{tabular}{>{\tiny}c|cccccc}
\hline
 & $K$ & $\sigma^2_{\bU}$ & $\sigma^2_{\bY}$ & $e_{\rm exact}$ & $e_{\rm GMM}$ & $e_{\rm BGMM}$\\
\hline
C1  & 500  & 0.005 & 0.0001 & 1.28e-01 & 2.80e-03 & 2.79e-03 \\
C2  & 500  & 0.01  & 0.0001 & 7.96e-02 & 2.25e-03 & 2.25e-03 \\
C3  & 500  & 0.05  & 0.0001 & 3.87e-01 & 1.30e-03 & 1.30e-03 \\
\hline
C4  & 5000 & 0.001 & 0.0001 & 2.86e-02 & 4.30e-03 & 3.77e-03 \\
C5  & 5000 & 0.005 & 0.0001 & 2.77e-02 & 2.00e-03 & 1.98e-03 \\
C6  & 5000 & 0.01  & 0.0001 & 6.45e-02 & 1.80e-03 & 1.78e-03 \\
\hline
C7  & 5000 & 0.005 & 0.001  & 2.90e-02 & 2.25e-03 & 1.97e-03 \\
C8  & 5000 & 0.005 & 0.01   & 4.40e-02 & 7.47e-03 & 1.63e-03 \\
C9  & 5000 & 0.005 & 0.1    & 2.60e-01 & 1.64e-01 & 1.13e-03 \\
\hline
\end{tabular}

\vspace{0.5em}
\captionof{table}{\footnotesize Comparison of $e_{\rm exact}$, $e_{\rm GMM}$ and $e_{\rm BGMM}$ varying $K$, $\sigma^2_{\bU}$ and $\sigma^2_{\bY}$ values. Note that $e_{\rm BGMM}$ contains error only from the time discretization of the reverse process (here we select $\Delta \tau = 10^{-3}$ for discretization of the pseudo-time domain). $e_{\rm GMM}$ contains time discretization error as well as the Bayesian error due to selection of the $\sigma^2_{\bY}$ parameter. $e_{\rm exact}$ contains error from the time discretization, Bayesian error, as well as error due to the number of available samples $K$. \textbf{Main observations}: 1. The error $e_{\rm BGMM}$ remains on the order of $10^{-3}$, and this low error is due to the time discretization scheme (rows 1-9). 2. The error $e_{\rm GMM}$ increases as $\sigma^2_{\bY}$ increases due to the smoothing effect of larger $\sigma^2_{\bY}$ values (rows 6-9). 3. As the number of samples \( K \) increases, the exact error \( e_{\mathrm{exact}} \) consistently decreases. Additionally, the $\sigma^2_{\bU}$  associated with the smallest error \( e_{\mathrm{exact}} \) decreases as $K$ increases, as can be observed in rows 2 and 5. This trend highlights the benefit of larger sample sizes combined with appropriately chosen prior variances in improving estimation accuracy. This trend can also be observed comparing row 2 (\( K = 500, \sigma^2_{\bU} = 10^{-2}, e_{\mathrm{exact}} = 7.96 \times 10^{-2} \)) with row 4 (\( K = 5000, \sigma^2_{\bU} = 10^{-3}, e_{\mathrm{exact}} = 2.86 \times 10^{-2} \)), which illustrates the reduction in error due to increased sample size and a corresponding decreased $\sigma^2_{\bU}$.}
\label{tab:full_comparison}
\end{center}

\begin{figure}[H]
    \centering
\includegraphics[width=0.8\linewidth]{ablation_studies/final_bimodal_plots.png}
\caption{\footnotesize Corresponding density plots to rows of Table \ref{tab:full_comparison}.The first row corresponds to rows 1-3, the second to rows 4-6, and the third to rows 7-9. In the first and second rows, $\sigma^2_{\bU}$ increases from left to right, revealing the effects of under- and over-smoothing in approximating the true conditional distribution. In the third row, we fix $\sigma^2_{\bU}$ and instead increase $\sigma^2_{\bY}$, illustrating how the posterior GMM begins to diverge from the exact conditional GMM. Increasing $\sigma^2_{\bY}$ results in over-smoothing when compared to the exact posterior.} %Blue histograms are the exact-score based diffusion model generated samples. The green line denotes the exact posterior. The blue line denotes the $p_{\rm BGMM}$ and the pink line denotes $p_{\rm GMM}$. Note $p_{\rm GMM}$ is distinguishable from $p_{\rm BGMM}$ only in rows 7-9 as we demonstrate the effects of increasing Bayesian error by increasing $\sigma^2_{\bY}$.}
    \label{fig:rows_of_table_comparisons1-3}
\end{figure}



% In the below table, we aim to analyze the effects of selecting a $\sigma^2_{\bV} \neq \sigma^2_{\bU}$. For each sample size $N$, we fix a $\sigma^2_{\bU}$ selected from the above table and fix $\sigma^2_{\bY} = 10^{-4}$:
% \begin{table}[H] 
% \centering
% \begin{tabular}{>{\tiny}c|cccccc}
% \hline
%  & $N$ & $\sigma^2_{\bU}$ & $\sigma^2_{\bV}$ & $e_{\rm exact}$ & $e_{\rm GMM}$ & $e_{\rm BGMM}$\\
% \hline
% % 0  & 500  & 0.001 & 0.0001 & 1.43e+00 & 1.75e+02 & 1.73e-02 \\
% 1  & 500  & 0.01 & 0.005 & 9.35e-02 & 2.36e-03 &2.34e-03 \\
% 2  & 500  & 0.01  & 0.01 & 7.96e-02 & 2.25e-03 & 2.25e-03 \\
% 3  & 500  & 0.01  & 0.05 & 1.92e-01& 1.72e-03 & 1.71e-03 \\
% \hline
% 4  & 5000 & 0.005 & 0.001 & 2.71e-02 & 2.12e-03 & 1.96e-03 \\
% 5  & 5000 & 0.005 & 0.005 & 2.77e-02 & 2.00e-03 & 1.98e-03 \\
% 6  & 5000 & 0.005  & 0.01 & 3.56e-02 & 2.06e-03 & 2.03e-03 \\
% \hline
% \end{tabular}
% \caption{Here we observe that selecting $\sigma^2_{\bV} \neq \sigma^2_{\bU}$ offers minimal or no improvement in error.}
% \end{table}



\subsubsection{Comment on time discretization error} \label{sec:time_error}

For all examples, we utilize the forward Euler method to solve the reverse diffusion process. We now demonstrate the expected linear convergence of $e_{\rm BGMM}$ when decreasing the time step size. We fix 10,000 initial conditions drawn from the normal distribution and vary the number time steps taken over the pseudo-time interval $[0,1]$. We fix $N = 5,000, \sigma^2_{\bY} = 0.0001, \sigma^2_{\bU} = \sigma^2_{\bV} = 0.005$. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{ablation_studies/Exact_Marginal_GMM_8to1024_final.png}

    \caption{Number of time-steps taken in the pseudo-time interval (ranging from 8 to 1024) vs. $e_{\rm BGMM}$. Note the expected linear convergence as the number of time-steps increases.}
    \label{fig:enter-label}
\end{figure}


% \subsubsection{Comment on selection of $\sigma^2_{\bU}$ and $\sigma^2_{\bV}$ based on mutual distance of joint samples}

% Consider the 500 prior data set. In the space of $\bU$ samples, after standardization of data, our data lies in the range of $m$. If we select $\sigma^2_{\bU} \propto (\frac{3.43}{N})^2$ for $\sigma^2_{\bU} \approx 4.64e-05$, note that this violates the "threshold" of distributions in which the Bayesian KL divergence is small. This is due to . Bayesian KL divergence for $N = 500, \sigma^2_{\bU} = 1e-4$ is 0.2945.  

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{ablation_studies/varU_0.0001_varV_0.0001_varY_0.0001_exact_conditional_500_samples.png}
%     \caption{$N = 500, \sigma^2_{\bU} = 1e-4, \sigma^2_{\bY} = 1e-4$}
%     \label{fig:enter-label}
% \end{figure}

% Considering the 5000 prior data set. In the space of $\bU$ samples, after standardization of data, can select $\sigma^2_{\bU} \propto (\frac{3.43}{N})^2$. Results in $\sigma^2_{\bU} \approx 4.7052e-07$ note that this violates the "threshold" of nice distributions in which Bayesian KL divergence is small. Bayesian KL divergence for $N = 5000, \sigma^2_{\bU} = 1e-4, \sigma^2_{\bY} = 1e-4$is 0.1059

% \begin{figure}[H]
%     \centering
% \includegraphics[width=0.5\linewidth]{ablation_studies/varU_0.0001_varV_0.0001_varY_0.0001_exact_conditional.png}
%     \caption{$N = 5000, \sigma^2_{\bU} = 1e-4, \sigma^2_{\bY} = 1e-4$}
%     \label{fig:enter-label}
% \end{figure}


% If we consider the average squared distance between joint sample and its nearest neighbor as a guide for parameter selection, we have an average distance of 0.001 for $N=500$. The average squared distance between joint sample and its nearest neighbor for the $N=5000$ dataset is 0.0001. 

% % \begin{table}[]
% %     \centering
% %     \begin{tabular}{c|c}
% %          &  \\
% %          & 
% %     \end{tabular}
% %     \caption{Caption}
% %     \label{tab:diff_v_values}
% % \end{table}


% % For $N=500$, this value is $\sim 10^{-3}$ while for $N=5000$, this value is $\sim 10^{-4}$. Due to the low-dimensionality of this illustrative problem, the choice of  $\sigma^2_{\bU}$ resulting in lowest $e_{\rm exact}$ error is larger than this baseline selection, as demonstrated in Table \ref{tab:full_comparison}. Hence we recommend beginning with this mutual distance, and incrementally increasing this value until distributions stablize.  

\subsection{20-Dimensional, 2-Mode GMM.}\label{sec:20D_2Mode_GMM}
In this example, we examine conditional distributions of a 20-dimensional, two mode GMM. We define the  two mode Gaussian Mixture as follows:
\begin{equation}
f(\bx) = \frac{1}{2}{\mathcal{N}}(\bx; \bmu_1, \mathbf{I}_{20}) + \frac{1}{2}{\mathcal{N}}(\bx; \bmu_2, \mathbf{I}_{20})
\end{equation}
where $\bmu_1 \in \mathbb{R}^{20}$ denotes the means of the first mixture component, $\bmu_2 \in \mathbb{R}^{20}$ the means of the second component, and we assume identity covariance matrices.   

We consider joint samples $\bX = [\bU, \bV]^{\top}$ consisting of observed and unobserved dimensions; let $\bU \in \mathbb{R}^{d_u}$ denote the unobserved dimensions of the GMM, and $\bV \in \mathbb{R}^{d_v}$ denote the observed dimensions. The mean vectors defining the GMM may be rewritten as $\bmu_1 = [\bmu^{u}_1, \bmu^{v}_1]^{\top}$ and $\bmu_2 = [\bmu^{u}_2, \bmu^{v}_2]^{\top}$. For observation $\by \in \mathbb{R}^{d_v}$, our target conditional distribution is the unobserved dimensions conditioned on the observed dimensions, which can be defined exactly as follows:  
\begin{equation} \label{exact_conditional_density_20D_GMM}
f_{\bU|\bY}(\bx) = w_1{\mathcal{N}}(\bx;\bmu^{u}_1|\bY, \mathbf{I}_{d_u}) + w_2{\mathcal{N}}(\bx; \bmu^{u}_2|\bY, \mathbf{I}_{d_u})
\end{equation} 
where, due to the assumed diagonal covariance, we have $\bmu^{u}_1|\bY = \bmu^{u}_1$ and $\bmu^{u}_2|\bY = \bmu^{u}_2$. The weights are determined by:
\begin{equation}
  {w}_i = \frac{0.5{\mathcal{N}}(\by|\bmu^v_i, \mathbf{I}_{d_v})}{0.5{\mathcal{N}}(\by|\bmu^v_1, \mathbf{I}_{d_v}) + 0.5{\mathcal{N}}(\by|\bmu^v_2, \mathbf{I}_{d_v})}. 
\end{equation}

We will obtain the high dimensional conditional distribution via the exact score-guided diffusion model. We first consider the case with 15 unobserved and 5 observed dimensions. %as well as the case $u = 10$ and $v = 10$. 
We define the components of the mean vectors as follows, 
\begingroup
\setlength{\abovedisplayskip}{7pt}
\setlength{\belowdisplayskip}{7pt}
\begin{align*}
(\bmu_1)_d &= 1.35, \quad (\bmu_2)_d = -1.35, \quad \text{for } d = 1, \dots, 5, \\
(\bmu_1)_d &= 0.5, \quad (\bmu_2)_d = -0.5, \quad \text{for } d = 6, \dots, 10, \\
(\bmu_1)_d &= 0.2, \quad (\bmu_2)_d = -0.2, \quad \text{for } d = 11, \dots, 15, \\
(\bmu_1)_d &= 0.1, \quad (\bmu_2)_d = -0.1, \quad \text{for } d = 16, \dots, 20.
\end{align*}
\endgroup

We consider a joint sample set of size $K=150,000$, $\{(\bu_{k}, \bv_{k})\}_{k=1}^K$. For this example, we select $\sigma^2_{\bY} = 10^{-5}$ and $\sigma^2_{\bU} = \sigma^2_{\bV} = 0.10$. 
To train the network, we generate $J = 30,000$ labeled data for dataset defined in Eq.~\eqref{eq:labeled_dataset}. The network is 2 layers with 50 neurons, trained using ADAM with standard MSE loss and a learning rate of $10^{-3}$ for 50,000 epochs. Using the network, we generate 5000 samples from the approximate target conditional distribution.

In Figure~\ref{fig:20D_KDE_estimates_15D_case}, we depict results for approximating three marginal distributions using the exact score-based diffusion model as well as the trained amortized inference network. These plots are obtained by projecting the generated samples onto the line connecting the means of the Gaussian components. We observe that in high-dimensions, the exact score-guided diffusion model is able to generate samples that capture the underlying bimodal behavior. The amortized inference network similarly captures this behavior, and once trained, is able to generate conditional densities for the given input condition. In Figure~\ref{fig:joint_marginals_15D}, we present randomly selected 2D joint marginals, which further demonstrate good agreement. We provide discrepancy evaluations between the true underlying density and the approximate density in Table~\ref{tab:KL_15D}, where we report the average KL divergence computed across the marginal distributions per dimension as well as the KL divergence after projecting down to the line connecting the mean components. The results demonstrate good agreement of our approximate density and true underlying density. We repeat the experiment using the same joint dataset for the case when $\bU \in \mathbb{R}^{10}$ and $\bV \in \mathbb{R}^{10}$,  and corresponding results are depicted in Figure~\ref{fig:20D_KDE_estimates_10D_case}, Figure~\ref{fig:joint_marginals_10D} and Table~\ref{tab:KL_10D}. Results demonstrate that the exact-score guided diffusion model and corresponding inference networks are able to obtain good approximations to multi-modal, high dimensional distributions. 

\noindent
\begin{minipage}{\textwidth}\label{fig:20D_KDE_estimates_15D_case}
\centering
\includegraphics[width=0.27\linewidth]{20D_GMM/dim15_final/joint_diag_density_20D_condition_0.0_dimension15.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim15_final/joint_diag_density_20D_condition_-0.5_dimension15.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim15_final/joint_diag_density_20D_condition_0.5_dimension15.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim15_final/joint_diag_density_20D_condition_0.0_dimension15_NN.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim15_final/joint_diag_density_20D_condition_-0.5_dimension15_NN.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim15_final/joint_diag_density_20D_condition_0.5_dimension15_NN.png}
% \vspace{0.5em}
    \captionof{figure}{\small Samples projected onto the line connecting mean components $\bmu_1$ and $\bmu_2$, given observations $\by = 0 \cdot \mathbf{1}_{15}$ (blue), $\by = -0.5 \cdot \mathbf{1}_{15}$ (purple), and $\by = 0.5 \cdot \mathbf{1}_{15}$ (red), where $\bu, \bv \in \mathbb{R}^{15}$. The top row shows samples generated by the diffusion model, and the bottom row shows samples generated by the trained amortized inference neural network (NN).}
\end{minipage}

\noindent
\begin{minipage}{\linewidth}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Discrepancy Type} & \textbf{$\by = 0.0$} & \textbf{$\by = -0.5$} & \textbf{$\by = 0.5$} \\
\hline
Projection KL (NN)         & 0.0130  & 0.0156 & 0.0256 \\
Avg. KL per dimension (NN) & 0.0040 & 0.0047 & 0.0049 \\
\hline
\end{tabular}
\captionof{table}{\small KL divergence between the true density and the amortized inference network generated density for different conditioning values for the $\by \in \mathbb{R}^{15}$ case.}
\label{tab:KL_15D}
\end{minipage}



\noindent
\begin{minipage}{\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{20D_GMM/dim15_final/2x3_2D_marginals_condition0_dim15_final.png}
    \captionof{figure}{\small Comparison of the randomly selected true joint marginal distributions (green) and the corresponding joint marginal prediction generated by the amortized inference network (blue) for the $\by = 0 \cdot \mathbf{1}_{15}$ case.}
    \label{fig:joint_marginals_15D}
\end{minipage}
\noindent
\begin{minipage}{\linewidth}
    \centering
\includegraphics[width=0.27\linewidth]{20D_GMM/dim10_final/joint_diag_density_20D_condition_0.0_dimension10.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim10_final/joint_diag_density_20D_condition_-0.5_dimension10.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim10_final/joint_diag_density_20D_condition_0.5_dimension10.png}
    
\includegraphics[width=0.27\linewidth]{20D_GMM/dim10_final/joint_diag_density_20D_condition_0.0_dimension10_NN.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim10_final/joint_diag_density_20D_condition_-0.5_dimension10_NN.png}
\includegraphics[width=0.27\linewidth]{20D_GMM/dim10_final/joint_diag_density_20D_condition_0.5_dimension10_NN.png}
    
    \captionof{figure}{\small Here we depict the samples projected onto the line connecting mean components $\bmu_1$ and $\bmu_2$ given the observation $\by = 0 \cdot \mathbf{1}_{10}$ (blue), $\by = -0.5 \cdot \mathbf{1}_{10}$ (purple) and $\by = 0.5 \cdot \mathbf{1}_{10}$ (red), where $\bu \in \mathbb{R}^{10}$ and $\bv \in \mathbb{R}^{10}$. Top row are samples generated by the diffusion model. Bottom row is samples generated by the trained amortized inference network.}
    \label{fig:20D_KDE_estimates_10D_case}
\end{minipage}

\noindent
\begin{minipage}{\linewidth}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Discrepancy Type} & \textbf{$\by = 0.0$} & \textbf{$\by = -0.5$} & \textbf{$\by = 0.5$} \\
\hline
Projection KL (NN) & 0.0516  & 0.0320 & 0.0304  \\
% Projection KL (Diffusion)  & 0.05629& 0.03966 & 0.05972 \\
Avg. KL per dimension (NN)           & 0.0045 & 0.0132 & 0.0160 \\
% Avg. KL per dimension (Diffusion)    & 0.01358 & 0.02097 & 0.02638 \\
\hline
\end{tabular}
\captionof{table}{\small KL divergence between the true density and the amortized inference network generated density for different conditioning values for the $\by \in \mathbb{R}^{10}$ case.}
\label{tab:KL_10D}
\end{minipage}

\noindent
\begin{minipage}{\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{20D_GMM/dim10_final/2x3_2D_marginals_condition0_dim10_final.png}
    \captionof{figure}{\small Comparison of the randomly selected true joint marginal distributions (green) and the corresponding joint marginal prediction generated by the amortized inference network (blue) for the $\by = 0 \cdot \mathbf{1}_{10}$ case.}
    \label{fig:joint_marginals_10D}
\end{minipage}

% Average squared L2 distance to closest neighbor: 8.125443665477436
% Median squared L2 distance to closest neighbor: 7.788569927215576
% Average squared L2 distance to closest neighbor (normalized by dimension): 0.40627218327387177
% Median squared L2 distance to closest neighbor (normalized by dimension): 0.3894284963607788

% V
% Average squared L2 distance to closest neighbor: 4.148194464228153
% Median squared L2 distance to closest neighbor: 3.8844984769821167
% Average squared L2 distance to closest neighbor (normalized by dimension): 0.27654629761
% Median squared L2 distance to closest neighbor (normalized by dimension): 0.25896656513

% U
% Average squared L2 distance to closest neighbor: 0.10918181268411999
% Median squared L2 distance to closest neighbor: 0.0754261240363121
% Average squared L2 distance to closest neighbor (normalized by dimension): 0.02183636253
% Median squared L2 distance to closest neighbor (normalized by dimension): 0.0150852248

% \begin{figure}[H]
%     \centering
% \includegraphics[width=0.32\linewidth]{20D_GMM/dim15/condY_0.5/1_index_condY_0.5_dim15_no_diffusion.png}
% \includegraphics[width=0.32\linewidth]{20D_GMM/dim15/condY_0.5/2_index_condY_0.5_dim15_no_diffusion.png}
% \includegraphics[width=0.32\linewidth]{20D_GMM/dim15/condY_0.5/3_index_condY_0.5_dim15_no_diffusion.png}
% \includegraphics[width=0.32\linewidth]{20D_GMM/dim15/condY_-0.5/1_index_condY_-0.5_dim15_no_diffusion.png}
% \includegraphics[width=0.32\linewidth]{20D_GMM/dim15/condY_-0.5/2_index_condY_-0.5_dim15_no_diffusion.png}
% \includegraphics[width=0.32\linewidth]{20D_GMM/dim15/condY_-0.5/3_index_condY_-0.5_dim15_no_diffusion.png}
%     \caption{Using the trained amortized inference network, we are able obtain conditional distributions for the given input observation. The first row depicts several marginal distributions for the conditional distribution given input observation $\bY = 0.5\cdot \bm{1}_{v=15}$, while the second row depicts several marginal distributions given $\bY = -0.5 \cdot \bm{1}_{v=15}$. }
%     \label{fig:20D_KDE_estimates_condY0.5_case15dim}
% \end{figure}

\subsection{Elliptic PDE.}
Our next example is a parameter recovery problem of the random permeability field parameterizing the following 2D elliptic PDE:
\label{sec:elliptic_PDE}
\begin{equation}\label{eq:elliptic_pde}
\begin{aligned}
     - \nabla \cdot \left(e^{k(x,y)} \nabla u \right) &= f, \quad (x,y) \in D \\
    u(x,y) &= 0, \quad (x,y) \in \partial D
\end{aligned}
\end{equation} 
where $D = [0,1]^2$ and $f = 1$. 
Assume the log-permeability field is the following random expansion:
\begingroup
\setlength{\abovedisplayskip}{7pt}
\setlength{\belowdisplayskip}{7pt}
\begin{equation} \label{eq:elliptic_pde_random_expansion}
    k(x,y) = \sum_{m=1}^M \sum_{l=1}^L b_{ml} \sin(2\pi mx) \sin(2\pi ly), \quad b_{ml} \sim \mathcal{N}(0,1/(m+l)),
\end{equation}
\endgroup
where we set $M=L=2$. The vector of random coefficients is denoted as $\mathbf{b} \in \mathbb{R}^{d}$ for $d=4$. We assume to have available noisy observations of the solution field at 10 random spatial locations in domain $D$. Denote the noisy observations as, 
\begingroup
\setlength{\abovedisplayskip}{7pt}
\setlength{\belowdisplayskip}{7pt}
\begin{equation}
    \hat{u}(x) = u(x)(1+\epsilon)
\end{equation}
\endgroup
where we consider relative noise  $\epsilon \sim \mathcal{N}(0,0.01)$. Let $\hat{\bu} \in \mathbb{R}^{N}$ denote the vector of noisy solution observations at $N$ locations. The goal of this example is to approximate $p(\mathbf{b}|\hat{\bu})$, the conditional distribution of coefficients given the noisy and sparse observations of the solution field.

To obtain joint samples, we randomly sample $K=5000$ sets of coefficients ${\mathbf{b}}$ from the multivariate normal distribution defined in Eq.~\eqref{eq:elliptic_pde_random_expansion}. Using these coefficients, we generate the solution data by solving Eq.~\eqref{eq:elliptic_pde} on a $32 \times 32$ mesh using a second order finite element method. We then randomly selected the $N=10$ spatial locations labeled in Fig.~\ref{fig:generated_samples_PDE_testcase1} to obtain the corresponding solution data $\hat{\bu}$. Our prior joint sample set is defined as $\mathcal{D}_{\rm prior} = \{(\mathbf{b}_{k}, \hat{\bu}_{k})\}_{k=1}^{K=5000}$. 
We utilize our joint sample set to define the prior GMM components, setting $\sigma^2_{\bU} = \sigma^2_{\bV} = 0.10$ and $\sigma^2_{\bY} = 10^{-5}$. We run the reverse diffusion process for 1000 time-steps. 

% Note the average squared $l_2$ distance between joint samples and the nearest neighbor is $\sim0.1$. We run the reverse diffusion process for 1000 time-steps. 

To train the inference network, the exact-score diffusion model is used to generate the a labeled dataset of size $J = 5000$ in Eq.~\eqref{eq:labeled_dataset}. This labeled dataset is then used to train a fully-connected, feed-forward neural network ${F}_\theta: \mathbb{R}^{10+4} \rightarrow \mathbb{R}^4$ which maps normal samples and observed solution data to samples from the posterior distribution of coefficient values. The network architecture is one layer with 100 neurons, trained using ADAM with standard MSE loss and a learning rate of $10^{-3}$ for 20,000 epochs. 

To demonstrate the accuracy of our method, we test on two different permeability fields and their corresponding noisy solution data, depicted in Fig.~\ref{fig:generated_samples_PDE_testcase1} and Fig.~\ref{fig:generated_samples_PDE_test_case2}. We present results generated by the amortized inference network and note that the trained network is capable of generating samples from the posterior densities of both test cases. 

% \begin{figure}[H]
%     \centering
% \includegraphics[width=0.6\linewidth]{elliptic_PDE_final/test_cases.png}
%     \caption{Ground truth permeability fields and corresponding solution fields. The red dots and indices indicate the $K=10$ randomly sampled solution locations. First row: Test case 1. Second row: Test case 2. }
%     \label{fig:test_cases_elliptic_pde}
% \end{figure}

After obtaining samples from $p(\mathbf{b}|\hat{\bu})$, we solve the PDE with the generated parameterizations and obtain solution values at the $N=10$ spatial locations. We present the point-wise signed relative error at several of these spatial locations in Figure~\ref{fig:signed_relative_error2} and compare to the prior model's signed relative error. We see a clear reduction in variance due to the conditioning data, as well as good agreement to the true ground truth solution values. 

%In Figure~\ref{fig:MSE_relative_error}, we compare the relative MSE of the generated permeability fields versus the true underlying permeability field, with the relative MSE of generated solution data with the true solution data. We see that while the permeability field error varies, the solution data error stays close to 0. Figure~\ref{fig:coefficient_posterior} presents the posterior of the coefficient distribution after conditioning on the given observed data. 

\vspace{0.5em}
\noindent
\begin{minipage}{\linewidth}
    \centering
 \includegraphics[width=\linewidth]{elliptic_PDE_final_draft/testcase1_final/test_case_1_samples.png}

    \captionof{figure}{\small Test case 1: Generated samples from the amortized inference network, including the sample closest to ground truth permeability field in the $l_2$ sense. First row: ground truth and generated permeability fields. Second row: ground truth and generated solution fields. Labeled numbers in the true solution field plot denote the sample locations of solution data $\hat{\bu} \in \mathbb{R}^{10}$.}
    \label{fig:generated_samples_PDE_testcase1}
\end{minipage}

\noindent
\begin{minipage}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{elliptic_PDE_final_draft/testcase2_final/test_case_2_samples.png}

    \captionof{figure}{\small Test case 2: Generated samples the amortized inference network, including the sample closest to ground truth permeability field in the $l_2$ sense. First row: ground truth and generated permeability fields. Second row: ground truth and generated solution fields. Labeled numbers in the true solution field plot denote the sample locations of solution data $\hat{\bu} \in \mathbb{R}^{10}$.}
    \label{fig:generated_samples_PDE_test_case2}
\end{minipage}

The diversity of the generated permeability fields, as depicted in Figure~\ref{fig:generated_samples_PDE_testcase1} for the first test case and in Figure~\ref{fig:generated_samples_PDE_test_case2} for the second test case, demonstrates the ability of our method to capture the uncertainty of the parameter estimation problem; the good agreement at the solution locations depicted in Figure~\ref{fig:signed_relative_error2} confirms our ability to generate samples that agree with the observed solution data. This point is further illustrated in Fig.~\ref{fig:MSE_relative_error}, where we compare the relative MSE error of the generated permeability fields  versus the relative MSE error of the  corresponding generated solution data. While the error of the solution fields is aggregated around 0, the error of the permeability fields spans a much larger range, demonstrating our ability to quantify uncertainty of the underlying permeability field given the available sparse and noisy solution data. 


\vspace{1.5ex}
\noindent
\begin{minipage}{\linewidth}
    \centering
\includegraphics[width=\linewidth]{elliptic_PDE_final_draft/signed_relative_error.png}
    \captionof{figure}{\small Signed relative error at 3 sample locations, where sample locations are depicted in Figure~\ref{fig:generated_samples_PDE_testcase1}. Left figures to the dash line are associated with test case 1 (magenta) and right figures with test case 2 (red). Blue histograms represent the signed relative error of the prior samples. Note the reduced variance compared to the prior, as well as the coverage of the true solution at the sampled locations.}
    \label{fig:signed_relative_error2}
\end{minipage}

\noindent
\begin{minipage}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{elliptic_PDE_final_draft/relatie_MSE.png}
    
    \captionof{figure}{\small The relative MSE of the generated solutions at the 10 locations versus the MSE relative error of the diffusion model's generated permeability fields. Test case 1 is represented by magenta and test case 2 is represented by red. We experiment with varying $\sigma^2_{\bY}$ parameter, where for both test cases, the first image we select $\sigma^2_{\bY} = 1e-5$ and in the second image $\sigma^2_{\bY} = 1$. Note that as we increase $\sigma^2_{\bY}$, the likelihood becomes less informative, leading to an over-smoothed posterior and larger mean squared error (MSE) values at the observed solution locations. Also observe the wide spread relative MSE error of the permeability fields indicates diverse sample generation, while the relative MSE error at the solution data locations aggregates about 0. This indicates we are able to capture the conditions of the solution data as well as the appropriate uncertainty about the underlying permeability field. }
    \label{fig:MSE_relative_error}
\end{minipage}

% \begin{figure}[H]
%     \centering
% \includegraphics[width=0.49\linewidth]{elliptic_PDE_final_draft/prior_joint_marginals_gridless_labeled_lower.png}
% \includegraphics[width=0.49\linewidth]{elliptic_PDE_final_draft/posterior_joint_marginals_gridless_labeled_lower_selected.png}
    
%     \caption{Test case 1 joint marginals: Blue figures denote the prior marginal and joint marginal distributions of the coefficients $b_{11}, b_{12}, b_{21},b_{22}$. Magenta histograms denote the posterior marginal and joint marginal distributions for test case 2. Note the change in the posterior distributions of the coefficients as a result of conditioning on observed solution field values. Our method is able to generate diverse set of coefficient samples that, when used to solve the underlying PDE, results in low error at observed solution field locations.}
%     \label{fig:MSE_relative_error}
% \end{figure}


\begin{figure}[H]
    \centering
\includegraphics[width=0.49\linewidth]{elliptic_PDE_final_draft/testcase2_final/prior_joint_marginals_gridless_labeled_lower.png}
\includegraphics[width=0.49\linewidth]{elliptic_PDE_final_draft/testcase2_final/posterior_joint_marginals_gridless_labeled_lower.png}
    
    \caption{\small Test case 2 joint marginals: Blue figures denote the prior marginal and joint marginal distributions of the coefficients $b_{11}, b_{12}, b_{21},b_{22}$. Red histograms denote the posterior marginal and joint marginal distributions. Note the change in the posterior distributions of the coefficients as a result of conditioning on observed solution field values. Our method is able to generate diverse set of coefficient samples that, when used to solve the underlying PDE, results in low error at observed solution field locations.}
    \label{fig:coefficient_posterior}
\end{figure}

\section{Conclusion} We have presented an exact score-guided diffusion model for generating samples from target conditional posterior distributions. We further propose the training of an amortized Bayesian inference network that generates samples from the posterior given an input condition, enabling efficient inference. Approximating high-dimensional and multi-modal conditional distributions remains a central challenge in the scientific community. In many real-world applications, we wish to sample from such complex distributions despite only having access to sparse prior datasets. By analytically deriving the score function under a Gaussian Mixture Model (GMM) prior, we are able to obtain a tractable approximation to the target conditional distribution. In our numerical studies, we assume spherical covariance structures and demonstrate successful uncertainty quantification in multi-modal synthetic settings as well as a parameter estimation task. As a direction for future work, we plan to explore anisotropic covariance structures to enable more tailored GMM components. Our analytically derived, training-free score function — combined with the amortized Bayesian inference network —offers a principled approach to score function approximation while simultaneously enabling efficient conditional sampling.


% \begin{figure}[H]
%     \centering
% \includegraphics[width=\linewidth]{elliptic_PDE_final/l2_relative_errors_final.png}
%     \caption{The $l_2$ relative error of the generated solutions at the 10 locations versus the $l_2$ relative error of the generated permeability fields. Test case 1 is represented by magenta and test case 2 is represented by red, and we present results from using the diffusion model directly as well as the amortized inference network. Note that the wide spread $l_2$ error of the permeability fields indicates diverse sample generation, while the $l_2$ error of the solution data at the 10 sampled locations aggregates about 0. This indicates we are able to capture the conditions of the solution data as well as capture the appropriate uncertainty about the underlying permeability field.}
%     \label{fig:l2_relative_error}
% \end{figure}


% \section{Surface quasi-geostrophic
% turbulence (SQG) model}\label{sec:ex3}

% In this task, we consider image data from the surface quasi-geotrophic turbulence model and perform an up-scaling conditional image generation task. We consider noisy $32 \times 32$ images as our conditional data. Our target resolution is $256 \times 256$ images. For this example, we utilize our exact score based diffusion model in conjunction with SLERP (spherical linear interpolation) in order to obtain samples from the desired conditional distribution $p(\theta_{H}|\hat{\theta}_{L})$.

% Let $\theta(x,y,z,t)$ denote the scaled potential temperature on the bounding surfaces $z = 0$ and $z = H$, where here we focus on data collected at $z = 0$. Denote the joint dataset of noisy high and low resolution images as $\{\hat{\theta}_{H}^{(i)}, \hat{\theta}_{L}^{(i)}\}_{i=1}^N$ for a prior joint sample set of size $N=500$. Specifically, we consider one percent relative noise of the high resolution image data, 

% \begin{equation}
%     \hat{\theta}_{H} = {\theta}_{H}(1+\epsilon) \quad \epsilon \sim \mathcal{N}(0,\sigma)
% \end{equation}

% for $\sigma = 0.01$. To obtain  $\hat{\theta}_{L}$, we down-sample the high-resolution, noisy image data via block averaging with a factor of 8, obtaining pixelated 256×256 images. The goal is to sample from the density $p(\theta_{H}|\hat{\theta}_{L})$. 

% We proceed by first encoding the high- and low-resolution images into a $4 \times 32 \times 32$ latent space (using pretrained VAE model which consists of down sampling factor of 8 and 4 channel latent space). In this space, our procedure for obtaining samples from the target distribution is as followss:
% \begin{enumerate}
%     \item Run the exact score-guided diffusion model with joint samples in latent space. 
%     \item Obtain the updated weights to the exact score function as pseudo-time $\tau \rightarrow 1$; rank the components by contribution to the score function. 
%     \item Select joint sample defining the highest weighted components, and perform SLERP to generate the latent space samples. 
% \end{enumerate}

% Specifically, we select the joint samples with the 3 largest weighted components within the score function computation at pseudo-time $\tau = 0.99$, indicating the posterior conditional density's regions of highest probability. We perform SLERP among these samples for obtaining latent space samples. These samples are then pushed through the decoder into high resolution space ($256 \times 256$) to obtain samples from the target conditional distribution $p(\theta_{H}|\hat{\theta}_{L})$. Parameters for the diffusion model used are set as $\sigma^2_{\bU} = \sigma^2_{\bV} = 0.1$ and $\sigma^2_{\bY} = 1e-5$ and solved for 1000 pseudo-time steps. 
% \newpage
% Two test cases are presented in Figure~\ref{fig:SQG_generated_samples}. We demonstrate the ability of this method to generate realistic high resolution $256 \times 256$ images based off the down-sampled condition data. To evaluate our method, we down-sample the generated image to the pixelated image and compute the relative MSE between the generated samples and the conditioning data. We observe small relative MSE, indicating good agreement to the conditioning data. We also generate a diverse set of images, each with low relative MSE, demonstrating our ability to quantify the uncertainty of the pixelated, low-resolution image in high-resolution space.
% \begin{figure}[H]
%     \centering
% \includegraphics[width=0.95\linewidth]{SQG/IMG_3922.png}
%     \caption{\small Two test cases. Reference refers to the down-sampled image. The reference image is encoded into latent space and used as condition data for the latent diffusion model. We include 3 cases for each test case of generated images and the corresponding relative MSE of the down-sampled image compared to the reference image. We observe variation in the generated SQG images while maintaining low relative MSE when down-sampled and compared to the image condition.}
%     \label{fig:SQG_generated_samples}
% \end{figure}

% %Average squared $l_2$ distance between the joint samples and closest neighbor (latent space): $\sim 1.30$.




% \begin{figure}[H]
%     \centering
% \includegraphics[width=0.5\linewidth]{IMG_7249.png}
%     \caption{Test sample in high resolution space $256\times256$. Top row: Downsampled 32 x 32 image. Left: Original image. Right: Output from VAE. Bottom row: High resolution 256 x 256 image. Left: Original image. Right: Output from VAE.}
%     \label{fig:SQG_test_sample}
% \end{figure}


% \subsection{SLERP Procedure for Labeled Data Generation}
% \begin{enumerate}
%     \item Run prior joint samples ($\bU$ samples are $256 \times 256$ images and $\bV$ are the corresponding $32 \times 32$ down-sampled images) through VAE to get the latent space representation.
%     \item Run the diffusion model in latent space to get "ranking" of most probable image samples given the condition data.
%     \item Select the top two ranked images samples and conduct SLERP to generate the labeled data. 
% \end{enumerate}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{SQG/log_weights.png}
%     \caption{Unnormalized log-weight values, ranked lowest to highest. Blue is at time t=0.001 and yellow is at time t=0.999. $\sigma^2_{\bU} = 0.1$.}
%     \label{fig:enter-label}
% \end{figure}

% \newpage
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{IMG_7249.png}
%     \caption{Left column: down-sampled conditional and ground truth conditional image data. Right column: Output from the VAE given ground truth inputs.}
    
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\linewidth]{SQG/top_log_probs.png}
%     \caption{Three most probable images given the down-sampled condition image data according to the log probabilities provided by diffusion model.}
    
% \end{figure}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.9\linewidth]{SQG/diffusion_results1.png}
% \vspace{-4mm}
% \includegraphics[width=0.9\linewidth]{SQG/diffusion_results2.png}
% \vspace{-4mm}
% \includegraphics[width=0.9\linewidth]{SQG/diffusion_results3.png}
% \caption{Diffusion model results for three different downsampled images. Reference image is output of the decoder given original 256x256 image.}
% \label{fig:enter-label}
% \end{figure}




% \subsubsection{10 Random Observations}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.49\linewidth]{elliptic_PDE/30x30/30x30_observations.png}
%     \caption{Test case. Observations. }
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\linewidth]{elliptic_PDE/30x30/example_samples_30x30.png}
%     \caption{8 generated permeability field samples and corresponding pressure fields. }
%     \label{fig:enter-label}
% \end{figure}




% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \hline
%         \textbf{Coefficient} & \textbf{True Value} & \textbf{Best Ptwise Approx} & \textbf{Mean Posterior Value} & \textbf{Sample STD} \\
%         \hline
%         $b_{1,1}$ & 0.670 & 0.889 & 0.982 & 0.059 \\
%         $b_{1,2}$ & -0.790 & -0.688 & -0.768 & 0.058 \\
%         $b_{2,1}$ & 0.489 & 0.687 & 0.701 & 0.050 \\
%         $b_{2,2}$ & -0.279 & -0.023 & -0.001 & 0.0539 \\
%         \hline
%     \end{tabular}
%     \caption{Estimated coefficients with their true values, best approximation (point-wise error) from sampled values, mean posterior values, and sampled standard deviations.}
%     \label{tab:coefficients}
% \end{table}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\linewidth]{elliptic_PDE/30x30/pointwise_std_clear_5000.png}
%     \caption{Pointwise standard deviation among 100 generated samples and the ten random sampling locations.}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{elliptic_PDE/exact_perm_field.png}
%     \includegraphics[width=0.5\linewidth]{elliptic_PDE/30x30/best_sampled_30x30.png}
%     \caption{Closest sample.}
%     \label{fig:enter-label}
% \end{figure}

% \newpage
% \subsubsection{$6 \times 6$ observations}

% \begin{itemize}
%     \item Joint samples are $\bX \in \mathbb{R}^{40}$
%     \item Fixed $\sigma_{\bX} = 0.01$ and $\sigma_{\bY} = 1e-5$
%     \item Ran reverse diffusion process for 1000 pseudo-time steps 
%     \item 5000 prior GMM components 
% \end{itemize}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\linewidth]{elliptic_PDE/6x6/4_sampled_perm_fields_K_6x6.png}
%     \caption{Test case. Example posterior samples. }
%     \label{fig:enter-label}
% \end{figure}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \hline
%         \textbf{Coefficient} & \textbf{True Value} & \textbf{Best Ptwise Approx} & \textbf{Mean Posterior Value} & \textbf{Sampled STD} \\
%         \hline
%         $b_{1,1}$ & 0.670 & 0.640 & 0.547 & 0.058 \\
%         $b_{1,2}$ & -0.790 & -0.556 & -0.516 & 0.052 \\
%         $b_{2,1}$ & 0.489 & 0.468 & 0.458 & 0.062 \\
%         $b_{2,2}$ & -0.279 & -0.3716 & -0.504 & 0.060 \\
%         \hline
%     \end{tabular}
%     \caption{Estimated coefficients with their true values, best approximation from sampled values, mean posterior values, and sampled standard deviations.}
%     \label{tab:coefficients}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{elliptic_PDE/6x6/pointwise_SD_5000.png}
%     \caption{Pointwise standard deviation among 100 generated samples.}
%     \label{fig:enter-label}
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\linewidth]{elliptic_PDE/30x30/pointwise_std_clear_5000.png}
%     \caption{Pointwise standard deviation.}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{elliptic_PDE/exact_perm_field.png}
%     \includegraphics[width=0.5\linewidth]{elliptic_PDE/6x6/6x6_best_approx.png}
%     \caption{Closest sample.}
%     \label{fig:enter-label}
% \end{figure}

